Cluster Aware Graph Anomaly Detection

Graph anomaly detection has gained significant attention across various domains, particularly in critical applications like fraud detection in e-commerce platforms and insider threat detection in cybersecurity. Usually, these data are composed of multiple types (e.g., user information and transaction records for financial data), thus exhibiting view heterogeneity. However, in the era of big data, the heterogeneity of views and the lack of label information pose substantial challenges to traditional approaches. Existing unsupervised graph anomaly detection methods often struggle with high-dimensionality issues, rely on strong assumptions about graph structures or fail to handle complex multi-view graphs. To address these challenges, we propose a cluster aware multi-view graph anomaly detection method, called CARE. Our approach captures both local and global node affinities by augmenting the graph's adjacency matrix with the pseudo-label (i.e., soft membership assignments) without any strong assumption about the graph. To mitigate potential biases from the pseudo-label, we introduce a similarity-guided loss. Theoretically, we show that the proposed similarity-guided loss is a variant of contrastive learning loss, and we present how this loss alleviates the bias introduced by pseudo-label with the connection to graph spectral clustering. Experimental results on several datasets demonstrate the effectiveness and efficiency of our proposed framework. Specifically, CARE outperforms the second-best competitors by more than 39% on the Amazon dataset with respect to AUPRC and 18.7% on the YelpChi dataset with respect to AUROC. The code of our method is available at the GitHub link: https://github.com/zhenglecheng/CARE-demo.

==> Theoretical_analysis.tex <==
\section{Theoretical Analysis}

In this section, we show some theoretical analyses regarding the regularization term $\mathcal{L}_c$.
% \subsection{How does $\mathcal{L}_c$ alleviate the issue of false positive sample?}
% \label{interpretation}
% In this subsection, we first show that $\mathcal{L}_c$ is a contrastive learning loss.


\subsection{Geometric Interpretation of $\mathcal{L}_c$}
\label{geometric_interpretation}
Following~\cite{DBLP:conf/icml/0001I20}, we analyze \method~ from the perspective of Alignment and Uniformity on the hypersphere. The authors of ~\cite{DBLP:conf/icml/0001I20} decompose the contrastive learning loss into $\mathcal{L}_{align}$ and $\mathcal{L}_{uniform}$: 
\begin{equation}
\begin{split}
    \mathcal{L}(\bm{\hat{z}}_i,\bm{\hat{z}}_j, C(i)) &= \mathcal{L}_{align} + \mathcal{L}_{uniform} \\
     % &=-\log\frac{sim(\hat{z}_i, \hat{z}_j)}{sim(\bm{\hat{z}}_i, \bm{\hat{z}}_j) + \sum_{k\neq j}sim(\bm{\hat{z}}_i, \bm{\hat{z}}_k)} \\
    & =-\log\frac{sim(\hat{z}_i, \hat{z}_j)}{\sum_{k=1}^n sim(\bm{\hat{z}}_i, \bm{\hat{z}}_k)} \\
\end{split}
\end{equation}
where $\mathcal{L}_{align}=-\log(sim(\hat{z}_i, \hat{z}_j))=-{\hat{z}_i \hat{z}_j^T}/\tau$ and $\mathcal{L}_{uniform}=\log\sum_{k=1}^n$ $sim(\hat{z}_i, \hat{z}_k)$ is the logarithm of an arithmetic mean of the radial basis function kernel (RBF) response. Similarly, \method~ can be decomposed into  $\mathcal{L}_{align}$ and $\mathcal{L}_{uniform}$ as follow.
\begin{equation}
\begin{split}
    \mathcal{L}_c(\bm{\hat{z}}_i,\bm{\hat{z}}_j, C(i)) &= \mathcal{L}_{align} + \mathcal{L}_{uniform} \\
     &=-\log \frac{\exp(2\bm{o}_{ij}\bm{\hat{z}}_i(\bm{\hat{z}}_j)^T/\tau)}{\Pi_{k=1}^n\exp((\bm{\hat{z}}_i(\bm{\hat{z}}_k)^T/\tau)^2)^{\frac{1}{n}}}
\end{split}
\end{equation}
where $\mathcal{L}_{align}=-\log(\exp(2\bm{o}_{ij}\bm{\hat{z}}_i\bm{\hat{z}}_j^T/ \tau) )=-2\bm{o}_{ij}\bm{\hat{z}}_i\bm{\hat{z}}_j^T/\tau$ and $\mathcal{L}_{uniform}=\log(\Pi_{k=1}^n\exp((\bm{\hat{z}}_i\bm{\hat{z}}_k^T/\tau)^2))^{\frac{1}{n}}$ is the logarithm of a geometric mean of the squared RBF response. As shown by~\cite{DBLP:conf/nips/ZhuSK21, DBLP:books/daglib/0068019}, the geometric mean helps smooth out the Gaussian noise and lose less information than the arithmetic mean, thus enjoying better performance.




% \begin{align}
%     \mathcal{L}_{uniform} &=\log(\Pi_{k=1}^n\exp((\bm{\hat{z}}_i\bm{\hat{z}}_k^T/\tau)^2))^{\frac{1}{n}} 
%     = \frac{1}{n} * \sum_{k=1}^n \log(\exp((\bm{\hat{z}}_i\bm{\hat{z}}_k^T/\tau)^2))
% \end{align}

% \begin{definition}
%     \label{definition_2}
%     Given a sample $\bm{x_i}$, we say sample $\bm{x_j}$ is a false positive sample of $\bm{x_i}$, if their optimal representations satisfy~ $e^{(\bm{z_i})^T\bm{z_j}/\tau} \approx 0$ for some small positive value $\tau$. Similarly, we say sample $\bm{x_j}$ is a true positive sample of $\bm{x_i}$, if their optimal representations satisfy $e^{(\bm{z_i})^T\bm{z_j}/\tau} > 1$ for some small positive value $\tau$; we say sample $\bm{x_k}$ is a true negative sample of $\bm{x_i}$, if their optimal representations satisfy $e^{(\bm{z_i})^T\bm{z_k}/\tau} \approx 0$ for some small positive value $\tau$.
% \end{definition}


% \begin{theorem}
% \textit{
% If $\bm{M}=\bm{S}^{1}$ is a one-layer graph pooling layer, the proposed $\mathcal{L}_c$ could alleviate the issue of the presence of false positive sample in the batch during training .}
% \end{theorem}

% \begin{proof}
%     In Lemma~\ref{lemma_1}, we have show that $\mathcal{L}_c$ is equivalent to $\mathcal{L}_f = -\sum_{i=1}^n\sum_{j=1}^n \log\frac{\exp(2\bm{o}_{ij}\bm{\hat{z}}_i\bm{\hat{z}}_j^T/\tau)}{\Pi_{k=1}^n \exp((\bm{\hat{z}}_i\bm{\hat{z}}_k^T/\tau)^2)^{1/n}}$. We rewrite $\mathcal{L}_f$ as folows:

% \begin{align}
%     \mathcal{L}_f &= \sum_{i=1}^n \sum_{i=k}^n (\bm{\hat{z}}_i\bm{\hat{z}}_k^T/\tau)^2 - \sum_{i=1}^n\sum_{j=1}^n 2\bm{o}_{ij}\bm{\hat{z}}_i\bm{\hat{z}}_j^T/\tau
% \end{align}
%     By taking the derivative of $\mathcal{L}_f$ with respect to $\bm{\hat{z}}_j$, we have
% \begin{align}
% \label{false_negative_11}
%     \nonumber \frac{\partial \mathcal{L}_f}{\partial \bm{\hat{z}}_j} &= \frac{1}{\tau} \sum_{i \neq j} 
% \end{align}
% \end{proof}
